CaRT: Certified Safety and Robust Tracking in Learning-based Motion Planning for Multi-Agent Systems

The key innovation of our analytical method, CaRT, lies in establishing a new hierarchical, distributed architecture to guarantee the safety and robustness of a given learning-based motion planning policy. First, in a nominal setting, the analytical form of our CaRT safety filter formally ensures safe maneuvers of nonlinear multi-agent systems, optimally with minimal deviation from the learning-based policy. Second, in off-nominal settings, the analytical form of our CaRT robust filter optimally tracks the certified safe trajectory, generated by the previous layer in the hierarchy, the CaRT safety filter. We show using contraction theory that CaRT guarantees safety and the exponential boundedness of the trajectory tracking error, even under the presence of deterministic and stochastic disturbance. Also, the hierarchical nature of CaRT enables enhancing its robustness for safety just by its superior tracking to the certified safe trajectory, thereby making it suitable for off-nominal scenarios with large disturbances. This is a major distinction from conventional safety function-driven approaches, where the robustness originates from the stability of a safe set, which could pull the system over-conservatively to the interior of the safe set. Our log-barrier formulation in CaRT allows for its distributed implementation in multi-agent settings. We demonstrate the effectiveness of CaRT in several examples of nonlinear motion planning and control problems, including optimal, multi-spacecraft reconfiguration.

==> sections/4_safety.tex <==
\section{Analytical Form of Optimal Safety Filter}
\label{sec_safety}
In this section, we propose an analytical way to design a safety filter that guarantees collision-free operations of the systems~\eqref{eqlagrange} and~\eqref{equnderactuated} when $d^{i} = 0$ and $\Gamma^{i} = 0$. The idea here can also be viewed as a generalization of the frameworks~\cite{glas,lagrangian_collision} to Lagrangian and general control-affine nonlinear systems, constructed on top of the end-to-end learned control policy augmented with an optimality guarantee of the analytical solution to our safety filter. Note that instead of the condition on the barrier function $\dot{\psi}\leq 0$ used in~\cite{glas,lagrangian_collision}, which makes all sublevel sets of a safe set to be invariant and thus can lead to conservative control inputs, we optimize it using a condition relaxed to $\dot{\psi}\leq \alpha(H)$ to increase the available set of control inputs~\cite{cbf_clf}, where $\psi$ is a safety function, $H$ is a safety function associated with $\psi$, and $\alpha:[0,a]\mapsto[0,\infty]$ is a class $\mathcal{K}$ function with $a >0$~\cite[p. 144]{Khalil:1173048}. 
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Safety Function for Multi-Agent Safety}
We use the following local safety function:
\begin{align}
    \label{safety_def}
    \psi^{i}(o^{i}) = -\log \prod_{j\in \mathcal{S}^i}h(p^{ij}),~h(p^{ij}) = \frac{\|p_{ij}\|_{\Xi}-(r_{s}+\Delta r_{s})}{r_{\mathrm{sen}}-(r_{s}+\Delta r_{s})}
\end{align}
where $p^{ij} = p^{j}-p^{i}$, $\mathcal{S}^i$ is the set of all the neighboring objects (\ie{}, agents and obstacles), $r_{s}$ is the minimal safe distance between $i$th agent and other objects, $r_{\mathrm{sen}}$ is the sensing radius, and $\Delta r_{s}$ is a positive scalar parameter to account for the external disturbance to be formally defined in Sec.~\ref{sec_robustness}. We use the weighted $2$-norm $\|\cdot\|_{\Xi}$ with the weight $\Xi\succ0$ to consider a collision boundary defined by an ellipsoid as in the case of UAVs with downwash effects in the $z$ direction. The parameters are selected to satisfy 
\begin{align}
    \sup_{\|p_{ij}\|\leq r_{\mathrm{sen}}}\|p_{ij}\|_{\Xi} \leq r_{\mathrm{sen}}\text{ and }r_{\mathrm{sen}}-(r_{s}+\Delta r_{s}) > 0
\end{align}
to ensure $\psi^{i}(o^{i}) \geq 0$ always when the distance to the $j$th object is less than the sensing radius $r_{\mathrm{sen}}$. Having a negative value of $h$ implies a safety violation. The idea for our safety filter is first to construct a safe target velocity given as follows, and then to track it optimally using the knowledge of Lagrangian systems and contraction theory:
\begin{align}
    \label{safe_velocity}
    v^{i}_s(o^{i}) = \alpha(H^{i}(o^{i}))\|\nabla_{p^{i}}\psi^{i}(o^{i})\|^{-2}\nabla_{p^{i}}\psi^{i}(o^{i})
\end{align}
where $H^{i}(o^{i})=\prod_{j\in \mathcal{S}^i}h(p^{ij})$ and $\alpha:[0,a]\mapsto[0,\infty]$ is a class $\mathcal{K}$ function with $a >0$. 
\begin{lemma}
\label{lemma_velocity}
Suppose that $\alpha$ of~\eqref{safe_velocity} satisfies $\alpha(s)\leq (N-1)/(-\log s+(N-1))$ for $s\in(0,1]$, where $N$ is the number of all the agents. The controller $v^{i}=v^{i}_s(o^{i})$ for the single integrator system $\dot{p}^{i} = v^{i},~i=1,\cdots,N$ renders the system safe, \ie{}, the interior of the following set, $\mathrm{Int}(\mathcal{C})$, is forward invariant:
\begin{align}
    \mathcal{C} = \left\{x^{1},\cdots,x^{N}\in\mathbb{R}^n\left|\prod_{i=1}^N\prod_{i<j\in\mathscr{N}^{i}}h(p^{ij})\prod_{i=1}^N\prod_{j\in\mathscr{M}^{i}}h(p^{ij})\geq0\right.\right\}
\end{align}
where $\mathscr{N}^{i}$ denotes the set of all the neighboring agents of the $i$th agent and $\mathscr{M}^{i}$ denotes the set of all the neighboring static obstacles of the $i$th agent.
\end{lemma}
\begin{proof}
The proof follows by showing that the following continuously
differentiable function $\psi:\mathrm{Int}(\mathcal{C})\mapsto\mathbb{R}$ is 
\begin{align}
    \label{def_psi_all}
    \psi(X) = -\log H(X) = -\log\prod_{i=1}^N\prod_{i<j\in\mathscr{N}^{i}}h(p^{ij})\prod_{i=1}^N\prod_{j\in\mathscr{M}^{i}}h(p^{ij})~~~~
\end{align}
is a reciprocal barrier function~\cite{cbf_clf}, where $X = \{x^{1},\cdots,x^{N}\}$. For a class $\mathcal{K}$ function $\alpha_{\log}:[0,1)\mapsto\mathbb{R}$ given as
$\alpha_{\log}(s) = 0$~(if $s = 0$) and $\alpha_{\log}(s) = (-\log s)^{-1}$~(otherwise), we have that $\psi(X) = 1/\alpha_{\log}(H(X))$. Also, applying the controller~\eqref{safe_velocity} to the single integrator system $\dot{p}^{i} = v^{i},~i=1,\cdots,N$ gives $\dot{\psi}=\sum_{i=1}^N{\nabla_{p^{i}}\psi^{i}(o^{i})}^{\top}v^{i}_s(o^{i}) = \sum_{i=1}^N\alpha(H^{i}(o^{i}))$ for $\psi^{i}(o^{i})$ given by~\eqref{safety_def}. Using the assumption of this lemma, we have $\dot{\psi}\leq\sum_{i=1}^N(N-1)/(-\log H^{i}(o^{i})+(N-1))\leq N(N-1)/(-\log \prod_{i=1}^N H^{i}(o^{i}))\leq N(N-1)\alpha_{\log}(H(X))$, which implies that $\psi$ is indeed a reciprocal barrier function as $\alpha_{\psi}(H(X))=N(N-1)\alpha_{\log}(H(X))$ is a class $\mathcal{K}$ function.
\end{proof}
\begin{remark}
The assumption of Lemma~\ref{lemma_velocity}, $\alpha(s)\leq (N-1)/(-\log s+(N-1))$ for $s\in(0,1]$, can be satisfied by many class $\mathcal{K}$ functions (\eg{}, we can easily verify that $\alpha(s)=\|x\|^n$ with $n\geq1$ always satisfy this assumption). Also, we can still use the safe velocity $v^{i}_s(o^{i}) = -k_p\nabla_{p^{i}}\psi^{i}$ proposed in~\cite{glas} because of the relation $\dot{\psi} = \sum_{i=1}^N-k_p^2\|\nabla_{p^{i}}\psi^{i}\| \leq \alpha(H)$ that holds for any class $\mathcal{K}$ function $\alpha$. Again, the purpose of Lemma~\ref{lemma_velocity} is just to relax the condition for safety from $\dot{\psi}<0$ to $\dot{\psi}\leq\alpha(H)$.
\end{remark}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Optimal Safety Filter for Lagrangian Systems}
\label{sec_optimal_safety}
Given the learned control policy $\tau_{\ell}^{i}(o^{i})$ of Sec.~\ref{sec_learned_policy} for the system~\eqref{eqlagrange}, we design a control policy $\tau_{s}^{i}$ processed by our proposed safety filter as follows:
\begin{align}
    \label{safe_control}
    \tau_{s}^{i}(o^{i}) =  \tau_{\ell}^{i}(o^{i})-  \begin{cases} 
   \frac{e^{i}_v(\tau_{\ell}^{i}(o^{i})-\bar{\tau}_{s}^{i})^{\top}e^{i}_v}{\|e^{i}_v\|^2} & \text{if $(\tau_{\ell}^{i}(o^{i})-\bar{\tau}_{s}^{i})^{\top}e^{i}_v > 0$} \\ 
    0 & \text{otherwise}
    \end{cases}~~~~
\end{align}
where $e^{i}_v=v^{i}-v^{i}_s(o^{i})$ for $v^{i}_s(o^{i})$ of~\eqref{safe_velocity}, $\bar{\tau}_{s}^{i}$ is given as
\begin{align}
    \bar{\tau}_{s}^{i}=M^{i}\dot{v}^{i}_s+C^{i}v^{i}_s+G^{i}+D^{i}-k_p\nabla_{p^{i}}\psi^{i}-k_vM^{i}e^{i}_v
\end{align}
with its arguments omitted for simplicity, and $k_p,k_v>0$ are some design parameters. The controller~\eqref{safe_control} is well-defined even with the division by $\|e^{i}_v\|$ because the relation $(\tau_{\ell}^{i}(o^{i})-\bar{\tau}_{s}^{i})^{\top}e^{i}_v = 0 \leq 0$ holds when $\|e^{i}_v\| = 0$.
We have the following theorem for the safety guarantee.
%Note that $k^{i}$ and $\dot{k}^{i}$ can be computed as
%\begin{align}
%    k^{i} = -k_p\frac{\Xi p_{ij}}{\|p_{ij}\|_{\Xi}(\|p_{ij}\|_{\Xi}-(r_{s}+\Delta r_{s}))}
%    \dot{k}^{i} = 
%\end{align}
\begin{theorem}
\label{thm_lagrangian_safe}
Consider the following optimization problem:
\begin{align}
    \label{eqopt_lag}
    &\tau^{i}_{\mathrm{opt}} = \mathrm{arg}\min_{\tau^{i}\in\mathbb{R}^n}\|\tau^{i}-\tau_{\ell}^{i}(o^{i})\|^2 \mathrm{~\st{}~}(\tau^{i}-\bar{\tau}_{s}^{i})^{\top}e^{i}_v \leq 0.
\end{align}
Suppose that the assumption of Lemma~\ref{lemma_velocity} on $\alpha$ of~\eqref{safe_velocity} holds and that there exists a control input $\tau^{i}$ that satisfies the constraint of~\eqref{eqopt_lag} for each $i$. The safety of the system~\eqref{eqlagrange} is then guaranteed when $d^{i}=0$ and $\Gamma^{i}=0$, \ie{}, all the agents will not collide with the other objects when there is no external disturbance. Also, the problem~\eqref{eqopt_lag} is always feasible and its optimal solution is given by~\eqref{safe_control}, thereby minimizing the deviation of the safe control input from the learned control input $\tau_{\ell}^{i}(o^{i})$.
\end{theorem}
\begin{proof}
Let us consider the following Lyapunov-type function:
\begin{align}
    \mathcal{V} = \psi(X)+\sum_{i=1}^N\frac{\|v^{i}-v^{i}_s(o^{i})\|_{M^{i}(p^{i})}^2}{2} = \psi(X)+\sum_{i=1}^N\frac{\|e^{i}_v\|_{M^{i}(p^{i})}^2}{2}
\end{align}
where $\psi$ is given in~\eqref{def_psi_all}, $v^{i}_s(o^{i})$ is given in~\eqref{safe_control}, and $e^{i}_v=v^{i}-v^{i}_s(o^{i})$. By the definition of $h$ given in~\eqref{safety_def}, the collision-free operation of the system~\eqref{eqlagrange} is guaranteed as long as $\psi^{i}$ of~\eqref{safety_def} is bounded. Taking the time-derivative of $\mathcal{V}$, we get
\begin{align}
    \dot{\mathcal{V}} =& \sum_{i=1}^N{k_p\nabla_{p^{i}}\psi^{i}}^{\top}v^{i}+{e^{i}_v}^{\top}M^{i}\dot{e}^{i}_v+\frac{1}{2}\|e^{i}_v\|_{\dot{M}^{i}}^2 \\
    =& \sum_{i=1}^N{k_p\nabla_{p^{i}}\psi^{i}}^{\top}v^{i}+{e^{i}_v}^{\top}(-M^{i}\dot{v}^{i}_s-C^{i}v^{i}_s-G^{i}-D^{i}+\tau^{i}) \\
    =& \sum_{i=1}^N{k_p\nabla_{p^{i}}\psi^{i}}^{\top}v^{i}_s-k_v\|e^{i}_v\|_{M^{i}}^2+(\tau^{i}-\bar{\tau}_{s}^{i})^{\top}e^{i}_v \label{last_eq}
\end{align}
by using~\eqref{eqlagrange} for $d^{i}=0$ and $\Gamma^{i}=0$ along with the relation $z^{\top}(\dot{M}^{i}-2C^{i})z=0,~\forall z\in\mathbb{R}^n$, where the arguments are omitted for notational simplicity. As seen in the proof of Lemma~\ref{lemma_velocity}, we have $\sum_{i=1}^N{k_p\nabla_{p^{i}}\psi^{i}}^{\top}v^{i}_s\leq k_p\alpha_{\psi}(H(X))$ for the first term of~\eqref{last_eq}, and thus, having $(\tau^{i}-\bar{\tau}_{s}^{i})^{\top}e^{i}_v$ as in the constraint of~\eqref{eqopt_lag} gives $\dot{\mathcal{V}}\leq k_p\alpha_{\psi}(H(X))-k_v\sum_{i=1}^N\|e^{i}_v\|_{M^{i}}^2$. Therefore, ({\color{red} I think this part is not true... may have to switch to $H^{i}$ with a Lyapunov function $V = -H+\mathcal{E}$. Question: If $\dot{B}+\dot{V}\leq \alpha(1/B)-2\beta V \Rightarrow B+V \leq 1/\sigma(1/B_0,t)+V_0e^{-2\beta t}?$ ($\alpha$: class $\mathcal{K}$ function, $\sigma$: class $\mathcal{KL}$ function, $\beta > 0$) $\Rightarrow$ this requires Lipschitz assumption, something like $\alpha(1/B)-\alpha(1/(V+B))\leq L V$}) the comparison lemma~\cite[pp. 102-103, pp. 350-353]{Khalil:1173048} used along with the Lemma~1 of~\cite{cbf_clf} and the Lemma~4.2~and~4.4 of~\cite[pp. 144-147]{Khalil:1173048} results in
\begin{align}
    H(X) \geq \alpha_{H}\left(\left(\frac{1}{\sigma_{H}\left(\frac{1}{\psi(X(0))},t\right)}+\sum_{i=1}^N\mathcal{E}^{i}(o^{i}(0))e^{-2k_v t}\right)^{-1}\right)    
\end{align}
for some class $\mathcal{K}$ function $\alpha_{H}$, class $\mathcal{KL}$ function $\sigma_{H}$, and $\mathcal{E}^{i}(o^{i}) = \sum_{i=1}^N\|e^{i}_v\|_{M^{i}}^2/2$ which implies no safety violation as long as the system is initially safe. Also, the constraint $(\tau^{i}-\bar{\tau}_{s}^{i})^{\top}e^{i}_v\leq0$ is always feasible for $\tau^{i}$ given as $\tau^{i}=\bar{\tau}_{s}^{i}$. Finally, applying the KKT condition~\cite[pp. 243-244]{citeulike:163662} to the optimization problem~\eqref{eqopt_lag} results in $\tau^{i}_{\mathrm{opt}}=\tau_{s}^{i}(o^{i})$ for $\tau_{s}^{i}(o^{i})$ given in~\eqref{safe_control}.
\end{proof}
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsection{Optimal Safety Filter for General Nonlinear Systems}
\label{sec_optimal_safety_general}
One way to generalize the results of Theorem~\ref{thm_lagrangian_safe} for nonlinear systems~\eqref{equnderactuated} is to construct a Lyapunov function, which can be used to track the safe velocity of~\eqref{safe_velocity}.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsubsection{Incremental Lyapunov Function}
\label{incremental_lyapunov}
We use the following incremental Lyapunov function inspired by contraction theory, which leads to a safety analysis analogous to that of linear time-varying systems and Lagrangian systems~\eqref{eqlagrange} as in~\cite{glas} and in Theorem~\ref{thm_lagrangian_safe}:
\begin{align}
    &\mathcal{E}^{i}(o^{i},t) = \frac{\|v^{i}-v^{i}_s(o^{i})\|_{M^{i}(p^{i},t)}^2}{2} \label{simple_lyapunov} \\
    &\text{\st{}~}\dot{M}^{i}+M^{i}A_{s}^{i}+{A_{s}^{i}}^{\top}M^{i}-2M^{i}B^{i}{R^{i}}^{-1}{B^{i}}^{\top}M^{i} \leq -2k_vM^{i} \label{simple_contraction}
\end{align}
where $M^{i}(p^{i},t)\succ0$, $k_v$ is a design parameter, and $A_{s}^{i}(o^{i},t)$ is a nonlinear state-dependent coefficient matrix for the system of~\eqref{equnderactuated} defined as follows:
\begin{align}
    \label{sdc_matrix}
    A_{s}^{i}(o^{i},t)(v^{i}-v^{i}_s(o^{i})) = f^{i}(p^{i},v^{i},t)-f^{i}(p^{i},v^{i}_s(o^{i}),t).
\end{align}
The arguments are omitted in~\eqref{simple_contraction} for notational convenience and the notations~\eqref{simple_lyapunov}~and~\eqref{simple_contraction} are intentionally consistent with the ones of Theorem~\ref{thm_lagrangian_safe} to imply the analogy between the methods in Sec.~\ref{sec_optimal_safety} and Sec.~\ref{sec_optimal_safety_general}. Note that the nonlinear matrix $A_{s}$ always exists when $f^{i}$ is continuously differentiable~\cite{nscm}.

The underlying benefit of using contraction theory here, in place of some other existing methods such as feedback linearization, is that the problem of finding $M^{i}$ in~\eqref{simple_contraction} can be expressed as a convex optimization problem for optimal disturbance attenuation~\cite{mypaperTAC}. Although we use one of the simple versions of a contraction metric in this paper for simplicity of discussion, we can consider more general types of Lyapunov functions and contraction metrics for the sake of the broader applicability of our approach by using, \eg{}, path integrals, geodesics, virtual systems, and differential dynamics, which allow for exploiting the linear time-varying systems-type techniques for nonlinear stability analysis and control/estimation synthesis. Reviewing how to find $M^{i}$ in~\eqref{simple_contraction} is beyond the scope of this paper, but those interested in knowing more about it can refer to~\cite{tutorial,chuchu_survey} and references therein.
%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%
\subsubsection{Augmenting General Learned Policy with Safety}
Let us first introduce the following assumption for generalizing the result of Theorem~\ref{thm_lagrangian_safe} using the Lyapunov function of Sec.~\ref{incremental_lyapunov}.
\begin{assumption}
\label{assump_natural}
Consider a Lyapunov-type function for~\eqref{equnderactuated} defined as follows:
\begin{align}
    \mathcal{V}^{i}(o^{i},t) = k_p\psi^{i}(o^{i})+\frac{\|v^{i}-v^{i}_s(o^{i})\|_{M^{i}(p^{i},t)}^2}{2}
\end{align}
for $k_p>0$, $\psi^{i}(o^{i})$ of~\eqref{safety_def}, $v^{i}_s(o^{i})$ of~\eqref{safe_velocity}, and $M^{i}(p^{i},t)$ of~\eqref{simple_contraction}. We assume that
\begin{align}
    \phi^{i}_v &= B(p^{i},v^{i},t)^{\top}\nabla_{v^{i}} \mathcal{V}^{i}(o^{i},t) = B(p^{i},v^{i},t)^{\top}M^{i}(p^{i},t)e^{i}_v = 0 \\
    &\Rightarrow\dot{\mathcal{V}}^{i}(o^{i},t) \leq k_p\alpha(H^{i}(o^{i}))-2k_v\mathcal{E}^{i}(o^{i},t) \label{safety_condition_i}
\end{align}
where $e^{i}_v=v^{i}-v^{i}_s(o^{i})$ for $v^{i}_s(o^{i})$ of~\eqref{safe_velocity}, $H^{i}(o^{i})$ is given in~\eqref{safety_def}, $\alpha$ is given in~\eqref{safe_velocity}, and $\mathcal{E}^{i}(o^{i},t)$ is given in~\eqref{simple_lyapunov}.
\end{assumption}

This assumption simply says that the system naturally satisfies the safety condition~\eqref{safety_condition_i} when the velocity displacements are in the directions orthogonal to the span of the actuated directions as discussed in~\cite{ccm}.
\begin{remark}
\label{remark_assumption}
Assumption~\ref{assump_natural} always holds for fully and over-actuated systems \st{} $B(p^{i},v^{i},t)B(p^{i},v^{i},t)^{\dagger} = \mathrm{I}_{n\times n}$, where $B(p^{i},v^{i},t)^{\dagger}$ the Moore-Penrose pseudo inverse of $B(p^{i},v^{i},t)$. This fact can be shown by observing that $B^{\top}M^{i}e^{i}_v = 0\Rightarrow v^{i}=v^{i}_s(o^{i})$ in this case. Furthermore, even when the system is underactuated and Assumption~\ref{assump_natural} does not hold, the error associated with the under-actuation can be treated robustly as to be seen in Sec.~\ref{sec_robustness}.
\end{remark}

Given the learned control policy $u_{\ell}^{i}(o^{i})$ of Sec.~\ref{sec_learned_policy} for the system~\eqref{equnderactuated}, we design a control policy $u_{s}^{i}$ processed by our proposed safety filter as follows:
\begin{align}
    \label{safe_control_general}
    u_{s}^{i}(o^{i}) = u_{\ell}^{i}(o^{i})-  \begin{cases} 
   \frac{\phi^{i}_v(u_{\ell}^{i}(o^{i})-\bar{u}_{s}^{i})^{\top}\phi^{i}_v}{\|\phi^{i}_v\|^2} & \text{if $(u_{\ell}^{i}(o^{i})-\bar{u}_{s}^{i})^{\top}\phi^{i}_v > 0$} \\ 
    0 & \text{otherwise}
    \end{cases}~~~~~
\end{align}
where $\bar{u}_{s}^{i}$ is given as
\begin{align}
    \bar{u}_{s}^{i }= 
    \begin{cases}
    \frac{\phi^{i}_v({e^{i}_v}^{\top}M^{i}(\dot{v}^{i}_s-f^{i}_s)-k_p{e^{i}_v}^{\top}\nabla_{p^{i}}\psi^{i})}{\|\phi^{i}_v\|^2} & \text{if $\|\phi^{i}_v\| \neq 0$}\\
    0 & \text{otherwise}
    \end{cases}
\end{align}
with $f^{i}_s=f^{i}(p^{i},v^{i}_s,t)$ and its arguments omitted for simplicity and with $k_p$ being a design parameter. The controller~\eqref{safe_control} is well-defined even with the division by $\|\phi^{i}_v\|$ because the relation $(u_{\ell}^{i}(o^{i})-\bar{u}_{s}^{i})^{\top}\phi^{i}_v = 0 \leq 0$ holds when $\|\phi^{i}_v\| = 0$. We have the following theorem for the safety guarantee.
\begin{theorem}
\label{thm_general_safe}
Consider the following optimization problem:
\begin{align}
    \label{eqopt_general}
    &u^{i}_{\mathrm{opt}} = \mathrm{arg}\min_{u^{i}\in\mathbb{R}^n}\|u^{i}-u_{\ell}^{i}(o^{i})\|^2 \mathrm{~\st{}~}(u^{i}-\bar{u}_{s}^{i})^{\top}e^{i}_v \leq 0.
\end{align}
Suppose that Assumption~\ref{assump_natural} and the assumption of Lemma~\ref{lemma_velocity} on $\alpha$ of~\eqref{safe_velocity} hold. Suppose also that there exists a control input $u^{i}$ that satisfies the constraint of~\eqref{eqopt_general} for each $i$. The safety of the system~\eqref{equnderactuated} is then guaranteed when $d^{i}=0$ and $\Gamma^{i}=0$, \ie{}, all the agents will not collide with the other objects when there is no external disturbance. Also, the problem~\eqref{eqopt_general} is always feasible and its optimal solution is given by~\eqref{safe_control_general}, thereby minimizing the deviation of the safe control input from the learned control input $u_{\ell}^{i}(o^{i})$.
\end{theorem}
\begin{proof}
Let us consider a Lyapunov-type function $\mathcal{V} = \psi(X)+\sum_{i=1}^N\mathcal{E}^{i}(o^{i},t)$, where $\psi$ is given in~\eqref{def_psi_all}, $v^{i}_s(o^{i})$ is given in~\eqref{safe_control}, and $\mathcal{E}^{i}(o^{i},t)$ is given in~\eqref{simple_lyapunov}. Using the relation~\eqref{simple_contraction} and Assupmption~\ref{assump_natural}, we have that
\begin{align}
    \dot{\mathcal{V}} \leq \sum_{i=1}^Nk_p\alpha(H^{i}(o^{i}))-2k_v\mathcal{E}^{i}(o^{i},t) +(u^{i}-\bar{u}_{s}^{i})^{\top}\phi^{i}_v \label{last_eq_general}
\end{align}
when $d^{i}=0$ and $\Gamma^{i}=0$ in~\eqref{equnderactuated} as in the proof of Theorem~\ref{thm_lagrangian_safe}, where $H^{i}(o^{i})$ is given in~\eqref{safety_def}, $\alpha$ is given in~\eqref{safe_velocity}, and $\mathcal{E}^{i}(o^{i},t)$ is given in~\eqref{simple_lyapunov}. The rest follows from the proof of Theorem~\ref{thm_lagrangian_safe} below~\eqref{last_eq}.
\end{proof}
\begin{remark}
The safety filter of Theorem~\ref{thm_general_safe} minimizes the deviation of the safe control input from the learned control input trained using the general system~\ref{equnderactuated}, which implies also that it instantaneously minimizes the contribution of the under-actuation error even when Assumption~\ref{assump_natural} does not hold. This error can be then treated robustly as discussed in Remark~\ref{remark_assumption}.
\end{remark}
